Pre-training Tasks for User Intent Detection and Embedding Retrieval in E-commerce Search

BERT-style models pre-trained on the general corpus (e.g., Wikipedia) and fine-tuned on specific task corpus, have recently emerged as breakthrough techniques in many NLP tasks: question answering, text classification, sequence labeling and so on. However, this technique may not always work, especially for two scenarios: a corpus that contains very different text from the general corpus Wikipedia, or a task that learns embedding spacial distribution for a specific purpose (e.g., approximate nearest neighbor search). In this paper, to tackle the above two scenarios that we have encountered in an industrial e-commerce search system, we propose customized and novel pre-training tasks for two critical modules: user intent detection and semantic embedding retrieval. The customized pre-trained models after fine-tuning, being less than 10% of BERT-base's size in order to be feasible for cost-efficient CPU serving, significantly improve the other baseline models: 1) no pre-training model and 2) fine-tuned model from the official pre-trained BERT using general corpus, on both offline datasets and online system. We have open sourced our datasets for the sake of reproducibility and future works.

==> 2-related_work.tex <==
% \section{Related Work}
% \label{sec:related_work}

% \subsection{BERT and Pretrain Tasks}
% \label{sec:related:bert}
% Recently, BERT(Bidirectional Encoder Representations from Transformers), a novel language representation model, introducing unsupervised pre-training techniques in large scale corpus such as Wikipedia, and has already created colossal amount of state-of-the-art models in NLP(natural language processing) tasks with just simply fine-tuning on specific domain.

% BERT designs MLM(masked language model) and NSP(next sentence prediction) as two major pre-training tasks. MLM facilitates context words to predict masked words, given model the generalization ability. And NSP mostly computes the similarity of two sentences, which gives model the prior knowledge of similarity between both tokens and sentences. And also, there are a lot of customized pre-training approach such as xx.

% \textbf{Pre-training tasks in e-commerce search}



% \subsection{Challenges in User Intent Detection}
% \label{sec:intro:intent}
% [Briefly introduce product category and the hierarchy] In JD.com, there are millions of items with thousands of product categories. Each item belongs to a corresponding product category. In addition, product categories are often presented as a hierarchical structure. In JD.com, there is a three-level hierarchical product category structure. Table ~\ref{table1} gives a statistics and shows an example of product categories.
% \begin{table}[]
% \centering
% \caption{Data statistics of product categories.}
% \label{table1}
% \resizebox{.95\columnwidth}{!}{
% \begin{tabular}{cccc}
% \cline{1-4}
% Level & 1 & 2 & 3  \\ 
% \cline{1-4}
% Number of product categories & 266 & 2307 & 20832 \\
% an example of product category & fresh & fruit & banana \\
% an example of item title & -- & -- & fresh organic bananas fresh fruit \\
% \cline{1-4}
% \end{tabular}}
% \end{table}

% [What is query intent detection?]
% In e-commerce search, the objective of query intent detection is to map a user's input query into some pre-defined product categories.

% [The difficulties and importance] Query intent detection is an important and challenging e-commerce search engine module. Queries are usually short, vague and suffer from the lack of data insufficiency for long tail queries. Moreover, queries often have multiple intents with large scale label set. For e-commerce search system, a query's relevant product categories perform in recall, relevance and ranking stage, usually served as an important feature. Therefore, it is of vital importance for search engine to map a query into some pre-defined product categories.

% In early works, some rule based methods~\cite{jansen2007determining,rose2004detection} focus on identifying characteristics of user queries or utilizing the knowledge of user behavior. However, such methods have low recall as these methods rely on a variety of hand-crafted rules. Many unsupervised methods based on query clustering have been popularly studied~\cite{ren2014heterogeneous,wang2009mining,radlinski2010inferring}, which focus on seeking a better interpretation for query intents by leveraging search log. Recently, deep learning approaches~\cite{hashemi2016query,kumar2019shareable,chen2019bert,liu2020deep} have been growing applied in query intent detection because of their better semantic representation than previous statistical methods. Broder \etal apply retrieval augmentation technique in query classification domain. ULMFiT proposes an effective transfer learning method that can be easily applied to any task in NLP~\cite{ULMFiT}. Skinner \etal introduce that kind of transfer learning approach into e-commerce search which uses items' title and products to do pre-training~\cite{xx}. However, they did not consider the distribution difference between the source and target domain, and their training data are somehow inaccurate.

% Recently, BERT based methods achieve amazing results in most NLP tasks~\cite{BERT}, including query classification and document classification. Chen \etal propose a joint intent and slot filling method based on BERT. SLIM proposes a Slot-Intent classifier to solve multiple intents within an utterance problem~\cite{xx}. However, the above methods trivially apply the original 12-layer BERT-base model as their pre-training model. Inspired by ~\cite{xx}, to better utilize the information of e-commerce items' title and product categories, we design a customized pre-training approach for e-commerce query classification. To the best of our knowledge, we are one of the first practical exploration of applying the customized BERT pre-training techniques in query intent detection domain.

% \subsection{Challenges in Semantic Retrieval}
% \label{sec:intro:retrieval}
% In last decade, representation-based model alone with Approximate nearest neighbor(ANN) search is widely adopted in search and recommendation area. Specifically, DSSM~\cite{huang2013learning} alike models are commonly used, which measure the similarity between the query and the product. Researchers improve them from several ways. One typical approach is identifying or generating hard-negative samples~\cite{li2021embedding,liu2021que2search}. Another way is capturing more semantics from query~\cite{zhang2020towards}, user behaviors~\cite{li2021embedding}, or different modals~\cite{liu2021que2search,zhuge2021kaleido} by increasing the model capability. Some of them benefit from the BERT-style models to learn trivial attentions in long text or different modals~\cite{li2021embedding,liu2021que2search,zhuge2021kaleido}. However, BERT suffers from the drawback of short text representation, which limits by its uni-gram word embedding. In e-commerce, query is usually short and finite. Thus, n-gram representation is still commonly used as supplementary. In this paper, we design a customised pre-train task, which inspired by Chang's work~\cite{chang2020pre}, to improve the text representation in both query side and item side. This work could be supplement to any existing model.


==> 4-system.tex <==
\section{System}
\label{sec:system}

\begin{itemize}
    \item Introduce our effort of serving transformer model online, by fewer layers, 
\end{itemize}
